Gauge/Gravity Duality: Recovering the Bulk from the Boundary using AdS/CFT

Motivated by the holographic principle, within the context of the AdS/CFT Correspondence in the large t'Hooft limit, we investigate how the geometry of certain highly symmetric bulk spacetimes can be recovered given information of physical quantities in the dual boundary CFT. In particular, we use the existence of bulk-cone singularities (relating the location of operator insertion points of singular boundary correlation functions to the endpoints of boundary-to boundary null geodesics in the bulk spacetime) and the holographic entanglement entropy proposal (relating the entanglement entropy of certain subsystems on the boundary to the area of static minimal surfaces) to recover the bulk metric. Using null and zero-energy spacelike boundary-to-boundary geodesic probes, we show that for classes of static, spherically symmetric, asymptotically AdS spacetimes, one can find analytic expressions for extracting the metric functions given boundary data. We find that if the spacetime admits null circular orbits, the bulk geometry can only be recovered from the boundary, down to the radius of null circular orbits. We illustrate this for various analytic and numerical boundary functions of endpoint separation of null and spacelike geodesics. We then extend our analysis to higher dimensional minimal surface probes within a class of static, planar symmetric, asymptotically AdS spacetimes. We again find analytic and perturbative expressions for the metric function in terms of the entanglement entropy of straight belt and circular disk subsystems of the boundary theory respectively. Finally, we discuss how such extractions can be generalised.

==> Holography_extra.tex <==
% To understand the physics of black holes, one needs to consider their geometry. The simplest type of black hole to consider is the $d+1$ dimensional Schwarzschild black hole, given by,
% 
% \be
% \label{Schwarz}
% ds^2=-f(r)\,dt^2+\dfrac{dr^2}{f(r)}+r^2d\Om^2_{d-1},
% \ee
% where
% \be
% f(r)=1-\left(\dfrac{r_+}{r}\right)^{d-2}\equiv\chi^2(r)
% \ee
% defines the red shift factor $\chi$.\\
% 
% The metric has a curvature singularity at $r=0$ and a coordinate singularity at $r=r_+$ which defines the horizon. The horizon radius is related to the mass $M$, at infinity by,
% 
% \be
% \label{shr}
% r_+^{d-2}=\dfrac{16\pi M}{(d-1)\A_{d-1}}
% \ee
% where $\A_{d-1}=2\pi^{d/2}/\G(d/2)$ is the area of a unit $d-1$ sphere. The black hole has horizon area in Planck units
% 
% \be
% \label{sbhA}
% A=\A_{d-1}r_+^{d-1}
% \ee
% 
% The horizon is not a mathematical singularity, which can be seen by taking the ``near horizon limit''. If we define
% 
% \be
% y=r-r_+\quad\text{where}\quad y\ll r_+
% \ee
% 
% To leading order near the horizon, $\chi^2(r)=(d-2)y/r_+$, and so the metric becomes,
% 
% \be
% ds^2=-\dfrac{d-2}{r_+}y\,dt^2+\dfrac{r_+}{d-2}\dfrac{dy^2}{y}+dx_idx_i
% \ee
% 
% where $dx_i$ is an element of length in the two dimensional plane tangent to the horizon. If we now define
% 
% \bea
% X^+&=&\rho e^\om=2\ds\sqrt{\dfrac{r_+y}{d-2}}\,e^{\frac{2r_+}{d-2}t}\nn
% X^-&=&-\rho e^{-\om}=-2\ds\sqrt{\dfrac{r_+y}{d-2}}\,e^{-\frac{2r_+}{d-2}t}
% \eea
% 
% we see that the metric becomes
% 
% \be
% ds^2=-dX^+dX^-+dx_idx_i
% \ee
% 
% which is the Minkowski metric in light cone coordinates. Now it is obvious that there is no curvature singularity at the horizon.\\
% 
% Consider the situation of a particle falling through the horizon into the black hole singularity. In Schwarzschild coordinates, it takes an infinite amount of time for a particle to cross the horizon, so an observer at $r=\infty$ will see the particle asymptotically approach the horizon. On the other hand, from the point of view of a freely falling observer in the same frame as the particle, there is nothing special about the horizon. This apparent contradiction in viewpoints is the first instance of the complementary nature of black holes concerning the decriptions of matter of external and infalling observers.\\

% To see their thermodynamic nature, one can consider the behaviour of quantum fields in the near horizon limit. If one uses heuristic arguments concernings the thermal density matrix of free bosinic fields using a semi-classical calculation, one arrives at a relationship for the proper temperature of an obverver at distance $\rho$,
% 
% \be
% T(\rho)=\dfrac{1}{2\pi\rho}
% \ee
% 
% Therefore, an observer outside a black hole but in the near horizon limit will detect a temperature inversely propertional to the distance from the horizon. Conversely, the temperature as measured by a distant observer asymptotically far from the black hole is given by the Hawking temperature
% 
% \be
% \label{TH}
% T_H=\dfrac{\kappa}{2\pi}
% \ee
% 
% where $\kappa=\frac{d-1}{2r_+}$ is the surface gravity of the black hole.\\
% 
% The motivation for black hole entropy comes from two black hole theorems: The ``area theorem''(\cite{Haw1}) and the ``no-hair theorem''(\cite{Haw2,Israel1,Israel2,Carter,Haw3,Wald}).\\
% 
% The area theorem states that (classically) \textit{the area of a black hole event horizon never decreases with time}:
% 
% \be
% dA\geq 0.
% \ee
% 
% For example, if a massive particle is thrown into a Schwarzchild black hole (see equation \eqref{Schwarz}), the mass $M$ of the black hole increases, and thus the area $A=16\pi M^2$ increases. We see an immediate analogy with the second law of thermodynamics, where
% 
% \be
% \label{2TD}
% dS\geq 0.
% \ee
% 
% The no-hair theorem states that \textit{A stationary black hole in $3+1$ dimensions is characterised by only three quantities: mass, angular momentum, and charge}. Thus there is a big constraint on the number of final states give some random collapsing matter, suggesting that black holes have a very low entropy, in contradiction with the second law of thermodynamics.\\

% The resolution to this constraction is that black holes carry entropy proprtional to the area of its every horizon (\cite{Bek1,Bek2,Bek3}). If we use the thermodynamic relation between mass (energy) and temperature
% 
% \be
% dM=T_HdS,
% \ee
% we have an expression for the Berkenstein Hawking entropy,
% 
% \be
% S_{BH}=\dfrac{A}{4},
% \ee
% where we have used equations \eqref{shr}, \eqref{sbhA} and \eqref{TH}.\\
% 
% Thus we see that black holes have a temperature $T_H$, and entropy $S_{BH}$ and radiate via a quantum process. This is known as Hawking radiation, and confirms that the entropy of black holes should be considered a genuine contribution to the total entropy of the universe, and so \eqref{2TD} only holds for the sum of black hole entropy and matter entropy.
% 
% \newpage
% 
% \subsection{Entropy Bounds}
% 
% 
% \textbf{The Susskind bound}\\ 



% \textbf{The Bekenstein bound}\\
% 
% Consider the situtuation of a matter systen falling into a black hole, its entropy is lost to an outside observer and converted into black hole entropy via its increase in mass. If one considers equation \eqref{2TD} to be universal, it must hold for an arbitrarily large initial matter entropy. But the black hole does not care about the entropy of the matter system, only its mass/energy. This suggests a universal bound on the entropy of matter systems in terms of thier extensive parameters. We can show that this bound can be calculated in arbitrary spacetime dimension $D$ via a classical analysis of the \textit{Geroch process}, where a system is dropped into the black hole near the horizon.\\
% 
% Consider a weakly gravitating stable thermodynamic system of total energy $E$. Let $R$ be the radius of the smallest $d-1$ sphere circumscribing the system. The smallest change in the mass of the black hole $\delta M$ is given by the redshifted energy of the matter system at a distance $R$ from the horizon (i.e. when the sphere touches the horizon). Using the metric given in \eqref{Schwarz}, the redshift factor near the horizon in tems of the proper length $l$, is given by
% 
% \be
% \chi(l)=\dfrac{d-2}{2r_+}l.
% \ee
% Then we have
% \be
% \delta M\leq E\chi(l)\mid_R=\dfrac{d-2}{2r_+}E\,R.
% \ee
% So from equation \eqref{TH}, the black hole entropy increases by
% \be
% \delta S_{BH}=\dfrac{dS_{BH}}{dM}\delta M=\dfrac{\delta M}{T_H}\leq 2\pi E\,R,
% \ee
% and so via the second law of thermodynamics,
% \be
% S_{\text{matter}}\leq2\pi E\,R.
% \ee
% This is the Bekenstein bound on matter entropy.\\
% 

% The Holographic Principle concerns the counting of degrees of freedom. If we consider a large region of space $\G$, we would like to determine the dimensoinality of the state space that lives within $\G$. To do this, we first have to define what we mean by ``degrees of freedom''.\\
% 
% The number of dgreesof freedom in a quantum-mechanical system, $N$, is given by the logarithm of the dimension $\N$ of its Hilbert space $\H$:
% \be
% \label{dof}
% N=\ln\,\N=\ln\dim(\H).
% \ee
% The number of bits of information, $n$, need to characterize a state is given by the formula
% \be
% N=n\ln2,
% \ee
% Thus a system with $10$ spins has $\N=2^{10}$ states, $N=10\ln2$ degrees of freedom, and can store $10$ bits of information.\\

% Now one can start to ask the question about how much information is required to specify a system contained within a specific region. This question pertains to any system and thus concerns the amount of complexity of a system with the framework of the most fundamental theory, namely a unified theory of quantum gravity. In a naive fashion, one can consider some local quantum field theory enclesed in some volume $V$. If one includes gravity, we may expect distances less than the Planck length, $l_P=1.6\times 10^{-33}$cm, unresolved by a thery of quantum gravity, and so we can consider a lattice of quantum oscillators in a Planck grid with one oscillator per Planck volume. Thus, the total number of oscillators is $V$, each with $p$ states, and so the dimensionality of such a system is given by
% \be
% \N\sim p^V,
% \ee
% and so from \eqref{dof}, we see that the total number of degrees of freedom
% \be
% N\sim V\ln p\gtrsim V.
% \ee 
% This result interprets the intuition that degrees of freedom are local in space, and so complexity grows with volume. It will be shown that for a theory which includes gravity, this is not the case.
% 
% Thermodynamic entropy has a statistical interpretation in terms of measuring the lack of knowledge we have about the details of the microscopic theory given a macroscopic theory. Given that all thermodynamic systems should be governed by the same underlying theory, the question about information of a system contained within a specific region can be recast in terms of its entropy, $S$. Namely: \textit{``What is the entropy of a system given that only the bounday area is specified?''}. Once the answer is known, we can use the Boltzmann formula for entropy, $S=\ln\,\N$, to find the number of states
% \be
% \N=e^S.
% \ee
% This question can be answered in the context of the shperical entropy bound given in equation \eqref{seb}. Given that this bound does not care about the underlying fundamental theory, and $S=S_{BH}$ saturates this bound, the number of degrees of freedom in a region bounded by a sphere of area $A$ is
% \be
% \label{h1}
% N=\dfrac{A}{4}.
% \ee
% 
% information contained within $G$ is somehow related to information on the boundary $\delta G$.
% 
% So, in this case, $N$ scales with $A$. This is in contradiction to the previous estimation for $N$ from a local field theory where $N$ scales with $V$. The resolution to this contradiction is that the inclusion of gravity provides a limit to the number of quantum states that can be formed (i.e before a black hole appears), and so in our previous argument we overcounted the number of degrees of freedom that can be used for generating entropy. Another argument that degrees of freedom are non-local come from quantum-mechanical unitarity. Unitarity preserves information, and if a system was conerted into a black hole, some of that information would be irretrievable if $N$ scaled with $V$ and not $A$. This lead 't Hooft\cite{Hol3} and Susskind\cite{Hol2} to give a ``holographic'' interpretation to equation \eqref{h1}.\\
% 
% \textbf{The Holographic principle} (initial formulation):\\
% 
% \textit{A region with boundary of area $A$ is fully decribed by no more than A/4 degrees of freedom, or about 1 bit of information per Planck area. A fundamental theory, unlike local field theory, should incorporate this counterintuitive result.}\\
% 
% \subsection{The Covariant Entropy Bound}
% 
% We can attempt to generalise \eqref{seb} to a bound on any spacelike surfaces, not just shperical. Unfortunately, through cosmological arguments and considering a spherical collapsing star, it was shown that this bound is violated\cite{Hol6,Hol7}. If fact, by looking at weakly gravitating systems and the arbitrary choice of time coordinate\cite{Hol8}, it can be shown that even \eqref{seb} cannot hold. This covariant nature of the laws of physics motivated Buosso\cite{Hol4,Hol9} to conjecture a \textit{covariant entropy bound}. In a $d+1$-dimensional Lorentzian spacetime $M$, the covariant entropy bound can be stated as follows:\\
% 
% \textit{Let $A(B)$ be the area of an arbitrary $d-1$ dimensional spacial surface $B$ (which need not be closed). A $d$ dimensional hypersurface $L(B)$ is called a light-sheet of $B$ if $L$ is generated by light rays which begin at $B$, extend orthoganally away from $B$ to a caustic (where the light rays intersect). Let $S$ be the entropy on any light-sheet of $B$. Then}
% \be
% S[L(B)]\leq\dfrac{A(B)}{4}.
% \ee
% 
% It was shown by Buosso that this bound indeed holds for multiple examples, including the situations that violated the spacial entropy bound. This bound motivates a reformulation of the holographic principle\cite{Hol9}:\\
% 
% \textbf{The Holographic principle}\\
% 
% \textit{The covariant entropy bound is a law of physics which must be manifest in an underlying theory. This theory must be a unified quantum theory of matter and spacetime. From it, Lorentzian geometries and and thier matter content must emerge in such a way that the number of independent quantum states describing the light-sheets of any surface $B$ is manifestly bounded by the exponential of the surface area}:
% \be
% \label{holpr}
% \N[L(B)]\leq e^{A(B)/4}.
% \ee
% 
% The holographic principle implies a radical reduction in the number of degrees of freedom we use to describe nature. It esxposes quantum field theory, which has degrees of freedom at every point in space, as a highly redundant effective description, in which the true number of degrees of freedom is obscured.
% 
% \subsection{The AdS/CFT Correspondence and the Holographic Principle}

%supergravity

% \be
% \label{nonbpsbrane}
% ds^2=-\dfrac{f_+(r)}{\sqrt{f_-(r)}}\,dt^2+\sqrt{f_-(r)}\,\sum_{i=1}^pdx^idx^i+f_-(r)^{-\frac{1}{2}-\frac{5-p}{7-p}}\left(\dfrac{dr^2}{f_+(r)}+r^2d\Om^2_{8-p}\right),
% \ee

% where $d\Om_{8-p}^2$ is the metric on a unit round $S^{8-p}$ sphere, and
% 
% \bea
% e^{2\Phi}&=&g_s^2f_-(r)^{\frac{p-3}{2}},\nn
% f_\pm(r)&=&1-\left(\dfrac{r_\pm}{r}\right)^{7-p},\nn
% N&=&\dfrac{(r_+r_-)^{\frac{7-p}{2}}}{d_pg_sl_s^{7-p}},\nn
% M&=&\dfrac{(8-p)r_+^{7-p}-r_-^{7-p}}{(7-p)(2\pi)^7d_pl_P^8}.
% \eea
% 
% where $l_P=g_s^{1/4}$ is the 10-dimensional Planck length, $M$ is the mass of the black hole solution, $g_s$ is the asymptotic string coupling constant and $d_p$ is the numerical factor,
% 
% \be
% d_p=2^{5-p}\pi^{\frac{5-p}{2}}\,\G\left(\frac{7-p}{2}\right).
% \ee
% When $r_+\geq r_-$, this solution is a black hole with a horizon at $r=r_+$ and a curvature singularity at $r=r_-$. When $r_+<r_-$ there is a timelike naked singularity which is not allowed by the cosmic censorship hypothesis\cite{Wald}. So for physical spacetimes, the condition that $r_+\geq r_-$ puts a bound on the mass of the black hole:
% 
% \be
% M\geq\dfrac{N}{(2\pi)^pg_sl_s^{p+1}},
% \ee
% which is the BPS bound required by the 10-dimensional supersymmetry of type IIB SUGRA.\\
% 
% When this bound is saturated (i.e. $r_+=r_-$), the solution is an exremal $p$-brane which is a half BPS object. The exremal solution is given by the metric:


We start by determining the proper length $\L$.
\bea
\L(J)&=&-2R\int^J_{\rho_0}\dfrac{r\,dr}{\ds\sqrt{(R^2+r^2)(r^2-J^2)}}\nn
&=&2R\,\ln\left(\dfrac{\sqrt{\r+R^2}+\sqrt{\r-J^2}}{\ds\sqrt{R^2+J^2}}\right)
\eea
Now we can determine $h(r)$, using equation \eqref{exhr} we have,
\be
\sqrt{h(r)} = \dfrac{1}{r\pi}\dfrac{d}{dr}\int^r_{\rho_0}\dfrac{J\L(J)}{\sqrt{J^2-r^2}}\,dJ=\dfrac{1}{r\pi}\dfrac{d}{dr}I(r)
\ee
where
\be
I(r)=\int_{\rho_0}^r\dfrac{2J\,dJ}{\ds\sqrt{J^2-r^2}}\,\ln\left(\dfrac{\sqrt{\r+R^2}+\sqrt{\r-J^2}}{\ds\sqrt{R^2+J^2}}\right)
\ee 
Integrating by parts \cite{integrals}, gives
\be
I(r)=\int_{\r}^{r^2}\dfrac{\sqrt{x-r^2}}{R^2+x}\,dx
+\int^{r^2}_{\r}\dfrac{\sqrt{x-r^2}}{\sqrt{\r-x}\,(\sqrt{\r-x}+\sqrt{\r+R^2})}\,\d x=I_1(r)+I_2(r)
\ee
where
\be
I_1(r)=-2\sqrt{\r-r^2}+2\sqrt{r^2+R^2}\,\mathrm{arctan}\left(\sqrt{\dfrac{\r-r^2}{R^2+r^2}}\right)
\ee
and
\be
I_2(r)=I_{21}(r)+I_{22}(r)+I_{23}(r)
\ee
where
\bea
I_{21}(r)=2\sqrt{\r-r^2},\quad I_{22}(r)=-\pi\,R\sqrt{\r+R^2},\nn
I_{23}(r)=\pi\,R\sqrt{r^2+R^2}-2\sqrt{r^2+R^2}\,\mathrm{arcsin}\left(\sqrt{\dfrac{\r-r^2}{\r+R^2}}\right)
\eea
and so
\bea
I(r)&=&2\sqrt{r^2+R^2}\,\mathrm{arctan}\left(\sqrt{\dfrac{\r-r^2}{R^2+r^2}}\right)-\pi\,R\sqrt{\r+R^2}+\pi\,R\sqrt{r^2+R^2}\nn
&&-2\sqrt{r^2+R^2}\,\mathrm{arcsin}\left(\sqrt{\dfrac{\r-r^2}{\r+R^2}}\right)\nn
&=&\pi\,R\sqrt{r^2+R^2}+\text{const.}\nn
\nn
\thus\sqrt{h(r)}&=&\dfrac{R}{r\pi}\dfrac{d}{dr}\pi\sqrt{r^2+R^2}\nn
\nn
h(r)&=&\left(1+\dfrac{r^2}{R^2}\right)^{-1}\quad\text{as expected}\nn
\eea



==> Null2.tex <==
\chapter{Extra bits}

\numberwithin{equation}{section}

\section{Solving for $f(r)$ using $\D t(\a)$ instead of $\D\p(\a)$}

In chapter \ref{Null}, I derived a formula (see equation \eqref{exfr}) for extracting the function $f(r)$ in the metric \eqref{sm}, given the location of the endpoints of boundary-to-boundary null geodesics $\D t(\D\p)$. One can use the same method to recover $f(r)$ using $\D t(\a)$ instead via the equation
\be
\D t(\a) = 2\int^{\infty}_{r_{min}(\a)}\dfrac{{\a}\,dr}{f(r)\sqrt{{\a}^2-V(r)}}
\ee 
where $\a=E/J$ parametrises the set of boundary-to-boundary null geodesics.

In this case, using the same inversion techniques, we have
\be
\label{exfr2}
V(r)\int^{\sqrt{V(r)}}_{1/R}\dfrac{\D t(\a)}{\sqrt{V(r)-\a^2}}\,d\a-2\int^{\sqrt{V(r)}}_{1/R}\D t(\a)\sqrt{V(r)-\a^2}\,d\a-\dfrac{\pi}{r}=0
\ee
where $V(r)=f(r)/r^2$ is the potential.

\textbf{Is this worth adding to the thesis? One can find both $\D t(\a)$ and/or $\D\p(\a)$ from $\D t(\D\p)$ using
\be
\dfrac{d\D\p(\D t)}{d\D t}=\a
\ee
so this inversion adds nothing new, although the derivation of \eqref{exfr2} requires an additional step or two. Is it worth adding as a footnote maybe?}

\section{Solving for $f(r)$ perturbatively}

Given a generic function $\D\p(\a)$ which describes a perturbed AdS spacetime, we can expand about the pure AdS solution $\D\p(\a)=\pi$ in a power series by introducing a parameter $\e>0$ such that
\be
\label{pertdp}
\D\p(\a)=\pi\sum_{n=0}^{\infty}a_n\e^n(\a^2-1/R^2)^{n/2}
\ee
where $a_0=1$.

From the energy equation of null geodesics
\be
\dot{r}^2+V(r)=\a^2
\ee
we have the boundary values $\a\tend\frac{1}{R}$ as $r\tend\infty$, and so equation \eqref{pertdp} has the correct boundary behaviour $\D\p(1/R)=\pi$, since all boundary null geodesics end at the anti-podal point.

Using the ratio test, the series \eqref{pertdp} is convergent for
\be
\label{dpcon}
\e<\dfrac{1}{\sqrt{\a^2-1/R^2}}\lim_{n\tend\infty}\left|\dfrac{a_n}{a_{n+1}}\right|\sim r_m(\a),
\ee
where $r_m(\a)$ is the minimum radius for boundary-to-boundary null geodesics. \textbf{I am unsure whether this limit is finite or not. Can i pick these constants $a_n$ to be whatever I like?}

We can then ansatz a power series solution
\be
\label{pertV}
V(r)=\sum_{n=0}^{\infty}\e^nV_n(r)
\ee
where we have expanded about the pure AdS spacetime $V_0(r)=\dfrac{1}{r^2}+\dfrac{1}{R^2}$ in powers of $\e$. To have the correct asymptotics, $V_n(r)\sim\O(1/r^n)$, where $n\geq 3$. \textbf{I am unsure about this last point.}

One can now solve for the the functions $V_n(r)$ by substituting both the ansatz into \eqref{exfr}, and solving order by order in powers of $\e$.

Substituting \eqref{pertdp} into \eqref{exfr} and solving the integral, we have
\be
\dfrac{\sqrt{\pi}}{2}\sum_{n=0}^{\infty}a_n\e^n\dfrac{\G(\frac{2+n}{2})}{\G(\frac{3+n}{2})}\left(V(r)-\frac{1}{R^2}\right)^{\frac{n+1}{2}}-\dfrac{1}{r}=0
\ee
Now subtituting in the series \eqref{pertV}, and performing a Taylor series expansion in $\e$ about $\e=0$ (\textbf{Am I allowed to do this Taylor series, how can I motivate this? It seems as though this is valid for any value of $\e$ so long as $V(r)$ and $\D\p(\a)$ converge. Then is it really a perturbative expansion?}), we have
\bea
V_1(r)&=&-\dfrac{\pi}{2}a_1\dfrac{1}{r^3}\nn
V_2(r)&=&\left(\dfrac{5\pi^2}{16}a_1^2-\dfrac{4}{3}a_2\right)\dfrac{1}{r^4}\nn
V_3(r)&=&-\pi\left(\dfrac{7\pi^2}{32}a_1^3-2a_1a_2+\dfrac{3}{8}a_3\right)\dfrac{1}{r^5}\nn
&\vdots&\nn
V_n(r)&\propto&\dfrac{1}{r^{n+2}},
\eea
and so
\be
\label{fpert}
f(r)=\dfrac{r^2}{R^2}+1+\sum_{n=1}^\infty b_n(a_1,a_2,\cdots,a_n)\dfrac{\e^n}{r^n}
\ee
This power series is convergent for
\be
\e<r\lim_{n\tend\infty}\left|\dfrac{b_n}{b_{n+1}}\right|,\quad\forall r.
\ee
The lowest upper bound on $\e$ is when $r$ is minimum. For boundary-to-boundary null geodesics, this occurs at $r=r_m$ where $r_m$ is the radius of null circular orbits. Null circular orbits exist for this space time when the potential $V(r)$ has a global maximum, and so
\bea
\dfrac{dV(r)}{dr}&=&0\nn
\thus\sum^\infty_{i=0}b_n(n+2)\dfrac{\e^n}{r^n}&=&0,\quad b_0=1
\eea
has at least one real solution $r=r_m$. \textbf{This is true at first order in $\e$, but I don't know if this is true in general}

\subsection{Comparing with the AdSBH solution}

The AdSBH in $d+1$ dimensions ($d>2$), has metric \eqref{sm}, where
\be
f(r)=\dfrac{r^2}{R^2}+1-\dfrac{r_+^{d-2}}{r^{d-2}}\left(1+\dfrac{r_+^2}{R^2}\right)
\ee
Comparing this with \eqref{fpert}, we can match the behaviour in $r$ by setting $b_{n\neq d-2}=0$. This is done by setting $a_{0<n<d-2}=0$ and picking $a_{n>d-2}$ such that $b_{n>d-2}=0$. \textbf{Is this reasonable?}. Then we have
\be
f(r)=\dfrac{r^2}{R^2}+1+b_{d-2}\dfrac{\e^{d-2}}{r^{d-2}}
\ee
where
\be
b_{d-2}=-a_{d-2}\sqrt{\pi}\dfrac{\G(\frac{d}{2})}{\G(\frac{d+1}{2})}.
\ee
Matching the coefficients, we have
\be
\label{mcoef}
\e=r_+\left(1+\dfrac{r_+^2}{R^2}\right)^{\frac{1}{d-2}}\quad\text{and}\quad a_{d-2}=\dfrac{1}{\sqrt{\pi}}\dfrac{\G(\frac{d+1}{2})}{\G(\frac{d}{2})}.
\ee
The other non-zero coefficients such that $b_{n\neq d-2}=0$ are $a_{p(d-2)}$ where $p\in\mathbb{N}$. The first few in the series are given by
\bea
a_{2(d-2)}&=&\dfrac{(1+2d)}{4}\dfrac{1}{\sqrt{\pi}}\dfrac{\G(\frac{2d-1}{2})}{\G(d-1)}\nn
a_{3(d-2)}&=&\dfrac{(10-28d+15d^2)}{8}\dfrac{1}{\sqrt{\pi}}\dfrac{\G(\frac{3d-3}{2})}{\G(\frac{3d-4}{2})}\nn
\vdots\nn
a_{p(d-2)}&=&P_{p-1}(d)\dfrac{1}{\sqrt{\pi}}\dfrac{\G(\frac{3+p(d-2)}{2})}{\G(\frac{2+p(d-2)}{2})},
\eea
where $P_{p-1}(d)$ is an order ${p-1}$ polynomial in $d$.

Now we can determine the range of $\a$ for which the expansion of $\D\p(\a)$ given in \eqref{pertdp} is convergent. Using \eqref{dpcon}, and substituting for the coefficients $\e$ and $a_{p(d-2)}$, we have the condition
\be
\a^2<\dfrac{1}{R^2}+\dfrac{1}{r_+^2}\left(1+\dfrac{r_+^2}{R^2}\right)^{\frac{2}{2-d}}\left(\lim_{p\tend\infty}\left|\dfrac{a_{p(d-2)}}{a_{(p+1)(d-2)}}\right|\right)^2.
\ee
If we let the leading order term in $P_{p-1}(d)$ be given by $C_{p-1}d^{p-1}$, then for $d>1$, the convergence condition reduces to
\be
\a^2<\dfrac{1}{R^2}+\dfrac{1}{r_+^2}\left(1+\dfrac{r_+^2}{R^2}\right)^{\frac{2}{2-d}}\dfrac{1}{d^2}\lim_{p\tend\infty}\left(\dfrac{C_{p-1}}{C_p}\right)^2.
\ee
We already know of a physical upper bound to $\a$ set by the radius of null circular orbits $r_m$. Null geodsics entering the region $r<r_m$ do not return to the boundary due to the presence of the singularity. In the specific case of the AdSBH, $r_m$ is determined by the the global maximum of the potential $V(r)=f(r)/r^2$, and so
\be
\dfrac{dV(r)}{dr}\Big|_{r=r_m}=0\quad\thus r_m=r_+\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{1}{d-2}
\ee
The value of $\a$ at $r=r_m$ is given by the energy condition
\bea
\a_m^2=V(r_m)&=&\dfrac{1}{R^2}+\left(\dfrac{d-2}{d}\right)\dfrac{1}{r_m^2}\nn
&=&\dfrac{1}{R^2}+\left(\dfrac{d-2}{d}\right)\dfrac{1}{r_+^2}\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{2}{2-d},
\eea
and so the range of $\a$ which parametrises null geodesics in a $d+1$ dimensional AdSBH is given by
\be
\dfrac{1}{R^2}\leq\a^2<\dfrac{1}{R^2}+\left(\dfrac{d-2}{d}\right)\dfrac{1}{r_+^2}\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{2}{2-d}.
\ee
And so, we see that the power series \eqref{pertdp} is convergent for the entire range of $\a$ when
\be
\lim_{p\tend\infty}\left(\dfrac{C_{p-1}}{C_p}\right)^2>d^2\left(\dfrac{d-2}{2}\right)\left(\dfrac{d}{2}\right)^\frac{2}{2-d},
\ee
and the convergence condition is satisfied over the partial range $1/R^2\leq\a^2\leq1/R^2+n^2/r_m^2$ when
\be
\lim_{p\tend\infty}\left(\dfrac{C_{p-1}}{C_p}\right)>n\,d\left(\dfrac{d}{2}\right)^\frac{1}{2-d}
\ee
where $0<n^2<\frac{d-2}{2}$. \textbf{I can't add anymore here since i do not have a general form for $C_p$, although checking the first few terms gives $C_p\sim q^{p},\,q>1$, and so the convergence condition becomes}
\be
n\lesssim\dfrac{d}{q}\left(\dfrac{d}{2}\right)^\frac{1}{d-2}
\ee

One can ask when the power series \eqref{pertdp} at first order is a good approximation to the whole function. This occurs when
\be
\e\sqrt{\a^2-\dfrac{1}{R^2}}\ll\dfrac{a_1}{a_2}.
\ee
For the case of the AdSBH, we find the power series up to order $\e^{d-2}$ is a good approximation to $\D\p(\a)$ over the partial range $1/R^2\leq\a^2\leq1/R^2+n^2/r_m^2$, when
\be
n\ll\left(\dfrac{\G(\frac{d+1}{2})\G(d-1)}{\G(\frac{2d-1}{2})\G(\frac{d}{2})}\dfrac{d}{1+2d}\right)^\frac{1}{2-d}\sim 1,\quad d>2.
\ee
This first order approximation never holds over the entire range of $\a$, since the upper bound of $\a$ never satisfies this condition.

\textbf{Alternatively, one can consider the partial range $1/R^2\leq\a^2\leq1/R^2(1+m^2)$, and use the condition
\be
\e^2\left(\a^2-\dfrac{1}{R^2}\right)\ll\left(\dfrac{a_{d-2}}{a_{2(d-2)}}\right)^{\frac{2}{d-2}}\sim 1,
\ee
to show that
\be
m^2\ll\dfrac{R^2}{r_+^2}\left(1+\dfrac{r_+^2}{R^2}\right)^{-\frac{2}{d-2}}
\ee
Thus for a small black hole where $r_+<R$, the range of $\a$ is larger than for a large black hole where $r_+>R$. This reflects the fact that for a large black hole, the geometry is more perturbed, so the expansion around AdS is only valid for a smaller range of $r$. I.e. a calculation using $V(r)=\a^2$ for $d=4$ gives
\be
r_+^2\left(1+\dfrac{r_+^2}{R^2}\right)\ll r^2<\infty
\ee
I am unsure whether this analysis is any better than the previous one, or whether I should include this bit on determining the range of validity at all?}

\section{Determining $\D t(\D\p)$ given $\D\p(\a)$}

Consider the function
\label{trdp}
\be
\D\p(\a)=\pi\left(1+A(\a^2-1/R^2)^{n/2}\right)
\ee
This is the form of the power series at first order given in the previous section, where $A$ is some constant.

Subtituting this into \eqref{exfr}, one has equation for determining the geometry $V(r)$ 
\be
\sqrt{V(r)-\dfrac{1}{R^2}}+\dfrac{A\sqrt{\pi}}{2}\dfrac{\G(\frac{2+n}{2})}{\G(\frac{3+n}{2})}\left(V(r)-\frac{1}{R^2}\right)^{\frac{n+1}{2}}-\dfrac{1}{r}=0.
\ee
For $n=-1$ and $k=\frac{A\pi}{2}$, we have
\be
V(r)=\dfrac{1}{R^2}+\dfrac{1}{r^2}+k^2-\dfrac{2k}{r}
\ee
This only satifies the asymptotics of AdS at $A=0$ and so the $n=-1$ boundary function cannot represent a perturbed AdS space.

For $n=-1/2$ and $p=\frac{A\sqrt{\pi}}{2}\frac{\G(3/4)}{\G(5/4)}$, we have
\be
V(r)=\dfrac{1}{R^2}+\dfrac{1}{r^2}+\dfrac{p^4}{2}\left(1-\sqrt{1+\dfrac{4}{p^2r}}\right)+\dfrac{p^2}{r}\left(2-\sqrt{1+\dfrac{4}{p^2r}}\right)
\ee
where we pick the sign of the root such that $V(\infty)=1/R^2$.

For $n=1$, we have
\be
\label{n1V}
V(r)=\dfrac{1}{R^2}+\dfrac{1}{2}\left(\dfrac{4}{A\pi}\right)^2\left(1-1\sqrt{1+\dfrac{A\pi}{r}}+\dfrac{A\pi}{2r}\right)
\ee
where we pick the sign of the root such that $V(\infty)=1/R^2$. \textbf{Is this good enough to be asymptotically AdS?}

For $n=2$, if we let $\Xi^2(r)=V(r)-1/R^2$, then $\Xi(r)$ is a solution of the cubic
\be
\dfrac{2A}{3}\Xi(r)^3-\Xi(r)-\dfrac{1}{r}=0
\ee

One can determine $\D t(\D\p)$ by inverting expression \eqref{trdp} for $\a$ and using equation \eqref{atodt} with the substitution $x=\frac{\D\p-\pi}{A\pi}$ to get
\be
\D t(\D\p)=\pi+A\pi\int^\frac{\D\p-\pi}{A\pi}_0\dfrac{dx}{\sqrt{x^{2/n}+1/R^2}}
\ee
For general $n$, the integral is a hypergeometric function. For $n=1$, we have
\be
\label{n1dtdp}
\D t(\D\p)=\pi+A\pi\mathrm{arsinh}\left(\dfrac{R}{A\pi}(\D\p-\pi)\right).
\ee
For $n=2$,
\be
\D t(\D\p)=\pi\left(1-2\dfrac{A}{R}\right)+2\sqrt{A\pi}\sqrt{\D\p+\pi\left(\dfrac{A}{R^2}-1\right)}
\ee
These boundary functions can be related to the first order approximation of the AdSBH solution in $d=n+2$ by  setting $A=\e^{d-2}a_{d-2}$ and using the values \eqref{mcoef}. For $d=3$,
\be
\D t(\D\p)=\pi+2r_+\left(1+\dfrac{r_+^2}{R^2}\right)\mathrm{arsinh}\left(\dfrac{R}{r_+}\left(1+\dfrac{r_+^2}{R^2}\right)^{-1}(\D\p-\pi)\right).
\ee
For $d=4$,
\be
\D t(\D\p)=\pi-\dfrac{3}{2}\dfrac{r_+^2}{R}\left(1+\dfrac{r_+^2}{R^2}\right)^2+\sqrt{3}r_+\left(1+\dfrac{r_+^2}{R^2}\right)\sqrt{\D\p-\pi+\dfrac{3}{4}\dfrac{r_+^2}{R^2}\left(1+\dfrac{r_+^2}{R^2}\right)^2}.
\ee
\textbf{This is nice to work out, but i'm not sure of their use. Maybe I can do some plots and check with the numerical result}

\subsection{Gaussian Bump}

In this section we want to examine how the behaviour of an anomolous piece of boundary field theory data is represented in the bulk geometry. To do this, we add a Gaussian ``bump'' to a boundary curve $\D t(\D\p)$ where the bulk geometry is already known. 

Consider the boundary function
\be
\D t(\D\p)=\pi+\mathrm{arsinh}(\D\p-\pi).
\ee
This has the correct AdS boundary behaviour where $\D t(\pi)=\pi$ and $\D t'(\pi)=1$, and where $\D t<\D\p$ for $\a>1$. This is a simplified version of equation \eqref{n1dtdp} where we have set the AdS radius $R=1$ and the constant $A=1/\pi$. The dual bulk geometry was solved in \eqref{n1V}, and for this simplified case is given by,
\be
\label{Vbump}
V(r)=9-8\sqrt{1+\dfrac{1}{r}}+\dfrac{4}{r}
\ee
Now we can modify $\D t(\D\p)$ by introducing a Gaussian $g(\D\p)$ centred around a point $\D\p=c>\pi$ such that
\be
\D t(\D\p)\tend\D t_g(\D\p)=\D t(\D\p)+g(\D\p)
\ee
which will induce a change in the bulk geometry $V(r)\tend V_g(r)$.

For $\D t_g(\D\p)$ to represent boundary data on an asymptotically AdS geometry $V_g(r)$, it must satify the same constraints as $\D t(\D\p)$. The constraint $\D t_g(\pi)=\pi$ implies 
\be
g(\pi)=0
\ee
We also have the relationship 
\be
\label{atodtg}
\D t_g'(\D\p)=\dfrac{1}{\a}
\ee
from \eqref{atodt}, which will be used to extract the function $\D\p_g(\a)$. Since $\a=1$ is the boundary null geodesic which does not enter the bulk, and so $\D\p_g(1)=\pi$, we require from \eqref{atodtg} that $\D t_g'(\pi)=1$, which implies 
\be
g'(\pi)=0.
\ee 
Since Gaussian's have a large fall-off, we can can get asymptotically close to this constraint. 

From the energy constraint \eqref{EC}, $\a$ must take values in the range $[1,\infty)$, this implies the constraint 
\be
-\D t'(\D\p)<g'(\D\p)<1-\D t'(\D\p),\quad\forall\D\p>\pi
\ee
To find $\D\p_g(\a)$ from the inverse function $\a(\D\p)$, we require $\a(\D\p)$ to be monotonically increasing. Combining this with the previous constraint implies the final constraint
\be
g''(\D\p)<-\D t''(\D\p),\quad\forall\D\p>\pi.
\ee
A particular function which satifies these constraints is given by (see fig.\ref{bump})
\be
\label{gfn}
g(\D\p)=\dfrac{1}{100}\left(e^{-20(\D\p-\frac{3}{2}\pi)^2}-e^{-20(\frac{\pi}{2})^2}\right).
\ee
\begin{figure}[h!t]
\label{bump}
\centering
\includegraphics[height=3in,width=5in]{bump}
\caption{Here is a graph of $\D t(\D\p)$ and a profile of the Gaussian bump function given by $100g(\D\p)+\pi$, where $g(\D\p)$ is given in \eqref{gfn} and is centred around $\D\p=1.5\pi$}
\end{figure}
\begin{figure}[h!t]
\label{bump1}
\centering
\includegraphics[height=3in,width=5in]{bump1}
\caption{Here are plots of $\D\p(\a)$ (blue) and $\D\p_g(\a)$ (red). Notice $\D\p(\a)=\D\p_g(\a)$ when $g'(\D\p)=0$}
\end{figure}
\begin{figure}[h!t]
\label{bumpV}
\centering
\includegraphics[height=3in,width=5in]{bumpV}
\caption{Here is a plot of $V_g(r)$ (blue) given in \eqref{Vbump} with the profile of the difference $V_g(r)-V(r)$ (red) magified 100x. The cusp at $r=0.35$ is not real and is only due to lack of data points.}
\end{figure}
\\
\\
Using \eqref{atodtg}, we can find $\D\p_g(\a)$ (see figure\ref{bump1}), and from this we can determine $V_g(r)$ (see fig.\ref{bumpV}) from \eqref{exfr}. We see that the location of the centre of the two bumps $r=r_g$ is determined by $\D\p(\sqrt{V(r_g)})=1.5\pi$.
\\
\textbf{Unfortunately, the effects on the spacetime geometry are tiny due to the restrictions on $g(\D\p)$. I also worry whether $V(r)$ is indeed asymptotically AdS. Although, if one were to add a bump to 'say' the AdSBH, the bump would also have to be tiny, since the boundary function $\D t(\D\p)$ will be similar to the one used in the above analysis. I don't know really what to do here}

==> Null_office.tex <==
\chapter{Recovering the Bulk I}
\label{Null}

In chapter \ref{background}, we motivated two main results using AdS/CFT, namely the existence of bulk-cone singularities, and the holographic interpretation of entanglement entropy. Using such results, it is natural to consider how much information of the bulk spacetime can be determined given boundary CFT data. This is motivated by the holographic principle (see chapter \ref{background}) which concludes that information in an enclosed volume is completely determined by its boundary degrees of freedom. More specifically, this and the remaining chapters will be concerned with the following question:

\textit{Given a $d$-dimensional boundary CFT where one has knowledge of the location of its singular boundary correlators and knowledge of its entanglement entropy for certain subsets of the boundary manifold, can one determine the bulk geometry of the $d+1$-dimensional perturbed asymptotically AdS spacetime dual to this CFT?}

In this chapter, we consider a limiting version of the above question, where one has knowledge of the location of the bulk-cone singularities only. To answer such a question, one must first build up the framework upon which the question is to be analysed. As was stated in section \ref{probulk}, bulk-cone singularities arise in boundary correlators when they are connected by type $\B$ boundary-to-boundary null geodesics, and so it is neccesary to describe the properties of such objects.

\section{Boundary-to-boundary null geodesics in asymptotically AdS spacetimes}
\label{btbngeo}

As with all problems in GR, we begin with a metric. We consider a minimal generalised version of the metric of AdS space in global coordinates (see equation \eqref{gads2}), which corresponds to a class of static, asymptotically AdS metrics with spherical symmetry, given in $d+2$-dimensions as
\be
\label{sm}
ds^2 = -f(r)\,dt^2 + \dfrac{dr^2}{f(r)} +r^2\,d\Om^{2}_d.
\ee
$f(r)$ is a well behaved real function of one variable and we recover AdS space when we set $f(r)=1+(r/R)^2$, where $R$ is the AdS radius. In general, this spacetime is asymptotically AdS, which requires the condition for $r\tend\infty$,
\be
\label{asymads}
f(r)\tend\dfrac{r^2}{R^2}+1+\O\left(\dfrac{1}{r^{d-1}}\right).
\ee
The main example of a solution to Einstein's equations which satisfy such a condition is the AdS black hole in $d+2$-dimensions, given in equation \eqref{AdSBH}.

To simplify the problem of solving for the null geodesic equations of motion, we use spherical symmetry to pick a particular spacial plane on which the null geodesics live. A helpful choice is the equatorial plane, where $\{\th_1,\th_2,\cdots,\th_d\}=\{\phi,\pi/2,\cdots,\pi/2\}$ (using the coordinate set given in \eqref{sads}). Then the equations of motion for $t$ and $\p$ yeild 2 constants of motion
\be
\dot{t}\,f(r) = E \quad\text{and}\quad r^{2}\dot{\p} = J.\quad\left(\dot{x} = \frac{\d x}{\d\lambda},\quad\text{where $\lambda$ is the affine parameter}\right) 
\ee
For null trajectories, $\d s = 0$, thus the equation of motion for $r$ is given by
\be
\dot{r}^2 = E^2 - \dfrac{f(r)\,J^2}{r^2}.
\ee
By redefining the affine parameter $J\la\tend\la$, we can just consider the ratio $\a = \frac{E}{J}$ to parametrise the null trajectories. Thus, the geodesic equations of motion become
\be
\label{ge}
\dot{t} = \dfrac{\a}{f(r)},\quad\dot{\p} = \dfrac{1}{r^2},\quad\dot{r}^2=\a^2-V(r),
\ee
where $V(r)=f(r)/r^2$ is the effective potential in the radial direction.

This gives us two equations of motion
\be
\dfrac{dt}{dr}=\dfrac{\a}{f(r)\sqrt{{\a}^2-V(r)}}\quad\text{and}\quad\dfrac{d\p}{dr}=\dfrac{1}{r^2\sqrt{{\a}^2-V(r)}}.
\ee

Now we can quantify the location of the singularities of the correlation functions in the CFT in terms of the boundary coordinates of the bulk metric. Considering the metric given by equation \eqref{sm}, we see that these quantities can be described in terms of a function $\D\p(\D t)$, where if $G(x,x')$ is some singular correlator on the equatorial plane between the points $x=(t,\p)$ and $x'=(t',\p')$, then $\D t=t'-t$ and $\D\p=\p'-\p$. Given that the quantities $\D\p$ and $\D t$ are also the location of the endpoints of boundary-to-boundary null geodesics of the bulk metric, one can also express them in terms of the geometry of the bulk. Thus using the null geodesic equations of motion, we have
\be
\label{dt}
\D t(\a) = 2\int^{\infty}_{r_{min}(\a)}\dfrac{{\a}\,dr}{f(r)\sqrt{{\a}^2-V(r)}},
\ee
and
\be
\label{dph}
\D\p(\a) = 2\int^{\infty}_{r_{min}(\a)}\dfrac{dr}{r^2\sqrt{\a^2-V(r)}},
\ee
where $\a=E/J$ parameterises the null geodisics, and $r_{min}(\a)$ is the minimum radius that the null geodesic, with angular momentum $J=E/\a$, reaches into the bulk. The factor of 2 comes from the fact that the null trajectory goes from the boundary, down to the mimimun value $r_{min}(\a)$, then back to the boundary at $r=\infty$. For AdS space where $f(r)=1+r^2/R^2$, integrals \eqref{dt} and \eqref{dph} can be solved to find that $\D t(\a)=R\pi$ and $\D\p(\a)=\pi$ with $r_{min}(\a)=1/\sqrt{\a^2-1/R^2}$. Thus all boundary-to-boundary null geodesics in AdS space with radius $R$ which start at the same point, end at the same point. The same will be shown not to be true for perturbed asymptotically AdS spacetimes.

Now we can quantify the distinction between Type $\A$ and Type $\B$ boundary-to-boundary null geodesics referred to in section \ref{probulk}. Type $\A$ geodesics sit on the boundary at $r=\infty$, and so from \eqref{ge} and condition \eqref{asymads}, we have $\a_\A=1/R$. For Type $\B$ geodesics, we have $\a_\B>1/R$ since $\dot{r}^2>0$. The upper bound on $\a_\B$ is set by the radius of null circular orbits, $r_m$, for which null geodesics going inside such a radius will not return to the boundary. $r_m$ is defined by the global maximum of the potential, i.e. where $r_m$ is the smallest real root of $V'(r)=0$. Then using \eqref{ge}, the upper bound is given by $\sqrt{V(r_m)}$, and so $\a_\B\in(1/R,\sqrt{V(r_m)})$. See figure \ref{BHplot} to see the trajectories of boundary-to-boundary null geodesics in a spacetime containing null circular orbits. Of course for spacetimes where the global maximum is infinity, such as AdS space, there is no upper bound on $\a_\B$.
\begin{figure}[h!t]
\centering
\label{BHplot}
\begin{tabular}{cc}
\begin{minipage}{200pt}
\centerline{\includegraphics[width=200pt]{BHnulldp}}
\end{minipage}
&
\begin{minipage}{250pt}
\centerline{\includegraphics[width=250pt]{BHnulldt}}
\end{minipage}
\end{tabular}
\caption{These are $2$-dimensional plots of boundary to boundary null geodesics in an AdS-black hole geometry with metric given by \eqref{sm} with $f(r)=1+r^2-0.1/r^2$, where $d-1$ angular directions have been projected out. To plot the null trajectories, the spacetime has been compactified using the coordinate transformation $r=\mathrm{tan}(\tilde{r})$, thus the boundary is a timelike cylinder with radius $\tilde{r}=\frac{\pi}{2}$. The left figure illustrates the quantity $\D t(\a)$ via projection of the null geodesics on the $r$-$t$ plane, where $\a=\frac{E}{J}$ parameterises the null curves. The right figure illustrates the quantity $\D\p(\a)$ via projection of the null geodesics on the $r$-$\p$ plane. The black curves are the Type $\A$ boundary null curve with $\a_\A=1$. The colour coding for for the Type $\B$ geodesics for different values of   $\a_\B$ is given by $\{1.3,1.7,1.85,1.87\}=\{$Red, Green, Blue, Purple$\}$. Notice all Type $\B$ curves go down to a minimum value $r_{min}(\a)$ before returning to the boundary.}
\end{figure}
\begin{figure}
\label{BHplotdtdp}
\centering
\includegraphics[height=2.5in,width=4in]{BHnulldtdp}
\caption{This is a plot of $\D t(\D\p)$ for the AdSBH given in \eqref{sm} with $d=3$ and $f(r)=1+r^2-\m/r^2$. The black curve $\D t=\D\p$ is the Type $\A$ boundary null geodesic. The blue curve represents the spacetime depicted in figure \ref{BHplot} whith $\m=0.1$. The purple, green and red curves correspond to $\m=0.2,0.05,\text{and}\,0.01$ repectively. We see that all curves converge to the AdS solution $\D t=\D\p=\pi$ as $\a\tend 1$, and that $\D t<\D\p$ for $\a>1$.} 
\end{figure}
Since $\a$ is purely a bulk quantity, expressions \eqref{dt} and \eqref{dph} do not yet provide a relationship between the data in the CFT and the geometry of the bulk. But it can be shown that one can relate the bulk quantity $\a$ with the boundary quantities $\D\p$ and $\D t$.

Starting with equations \eqref{dt} and \eqref{dph}, one can take a derivative with respect to $\a$, yeilding the expressions
\be
\label{dadt}
\D t'(\a)=-\dfrac{2r_{min}'(\a)\,\a}{f(r_{min}(\a))\sqrt{\a^2-V(r_{min}(\a))}}+2\int^{\infty}_{r_{min}(\a)}\left(\dfrac{\a}{f(r)\sqrt{{\a}^2-V(r)}}\right)'\,dr,
\ee
and
\be
\label{dadph}
\D\p'(\a)=-\dfrac{2r_{min}'(\a)}{r_{min}(\a)^2\sqrt{\a^2-V(r_{min}(\a))}}+2\int^{\infty}_{r_{min}(\a)}\left(\dfrac{1}{r^2\sqrt{{\a}^2-V(r)}}\right)'\,dr,
\ee
where primed functions are partial derivatives with respect to $\a$. We have utilised the Leibnitz rule where if $a(\a), b(\a), c(\a,r)$ are continuous, well behaved functions, then
\bea
a(\a)&=&\int^{\infty}_{b(\a)}c(\a,r)\,dr\nn
\thus a'(\a)&=&-b'(\a)\,c(\a,b(\a))+\int^{\infty}_{b(\a)}c'(\a,r)\,dr.
\eea
The first terms in equations \eqref{dadt} and \eqref{dadph} are singular from the definition of $r_{min}(\a)$. But we know that $\D t'(\a)$ and $\D\p'(\a)$ are non-singular since the functions $\D t(\a)$ and $\D\p(\a)$ are well behaved within the range of $\a$. So we must be able to remove the singular pieces using a term inside the integrals. Taking the derivative in the second term of \eqref{dadph} and noting that $V(r_{min}(\a))=\a^2$, we find that
\be
\D\p'(\a)=-\dfrac{2\,r_{min}^{\prime}(\a)}{r^2_{min}(\a)\sqrt{\a^2-V(r_{min}(\a))}}-V'(r_{min}(\a))\,r_{min}'(\a)\int^{\infty}_{r_{min}(\a)}\dfrac{dr}{r^2(\a^2-V(r))^{\frac{3}{2}}}.
\ee
Integrating by parts gives us
\bea
\D\p'(\a)&=&-\dfrac{2\,r_{min}^{\prime}(\a)}{r^2_{min}(\a)\sqrt{\a^2-V(r_{min}(\a))}}-V'(r_{min}(\a))\,r_{min}'(\a)\left[\dfrac{2}{r^2V'(r)}\dfrac{1}{\sqrt{\a^2-V(r)}}\right]^{\infty}_{r_{min}(\a)}\nn
&&+V'(r_{min}(\a))\,r_{min}'(\a)\int^{\infty}_{r_{min}(\a)}\dfrac{d}{dr}\left(\dfrac{1}{r^2V'(r)}\right)\dfrac{dr}{\sqrt{\a^2-V(r)}}\nn
\nn
&=&2\,\a\int^{\infty}_{r_{min}(\a)}\dfrac{d}{dr}\left(\dfrac{1}{r^2V'(r)}\right)\dfrac{dr}{\sqrt{\a^2-V(r)}},
\eea
where we have used the fact that $\frac 1 2 \,V'(r_{min}(\a))\,r_{min}'(\a)=\a$.

A similar calculation for $\D t'(\a)$ gives us
\be
\D t'(\a)=2\int^{\infty}_{r_{min}(\a)}\dfrac{d}{dr}\left(\dfrac{1}{r^2V'(r)}\right)\dfrac{dr}{\sqrt{\a^2-V(r)}}.
\ee
This allows us to write
\be
\D\p'(\a)=\a\,\D t'(\a),
\ee
which can be rewritten in terms of the function $\D t(\D\p)$ as
\be
\label{atodt}
\dfrac{d\D t(\D\p)}{d\D\p}=\dfrac{1}{\a}.
\ee
For Type $\A$ geodesics, we know that $\a_\A=1/R$, and so using \eqref{atodt} we have $\D t_\A(\D\p_\A)=R\D\p_\A$. Note that $\D t_\A(\pi)=R\pi$, which is consistent with the pure AdS result. For Type $\B$ geodesics, $\a_\B>1/R$, and so $\D t_\B<R\D\p_\B\,\forall\,\a_\B$ (see figure \ref{BHplotdtdp}). 

Through equation \eqref{atodt}, we have found a way to relate the bulk parameter $\a$ to the boundary parameters $\D\p$ and $\D t$, and so equations \eqref{dt} and \eqref{dph} indeed become relationships between purely bulk data and purely boundary data. Thus these are the equations we need to use to find an expression for $f(r)$ and thus the metric itself.

\section{Solving for the metric}

Given that we know $\D t(\a)$ and $\D\p(\a)$ from the boundary data, we can now proceed to solve for $f(r)$ given equation \eqref{dph}\footnote{one can equally well use equation \eqref{dt} for this purpose but \eqref{dph} is a slightly simpler expression so we will choose this one}.

The extraction of $f(r)$ is complicated by the fact that equation \eqref{dph} is non-linear in $f(r)$. Non-linearity in any type of equation makes finding an analytical solution much harder, so it would be useful to find a quantity which is linear in the integrand and invert that instead. This can be done by identifying a linear equation which control the trajectory of the null geodesics. Such an equation is the ``energy equation'' taken from \eqref{ge}
\be
\label{EC}
\dot{r}^2+V(r)=\a^2.
\ee
Instead of integrating over the variable $r$, let us perform a substitution to integrate over the variable $V=V(r)$ instead. If we let $r_{min}(\a) = x$, we see an immediate simplification for the expression of $\D\p(\a)$,
\be
\D\p\left(\sqrt{V(x)}\right)=2\int^{\infty}_x\dfrac{\d r}{r^2\sqrt{V(x)-V(r)}}.
\ee
Now if we perform the substitution $V(r)=V$, and integrate over $V$, we have
\be
\D\p\left(\sqrt{V(x)}\right) = \int^{V(x)}_{V(\infty)}\dfrac{p(V)\,dV}{\sqrt{V(x)-V}},\quad\text{where}\quad p(V)=-2\,\dfrac{dr(V)}{dV}\dfrac{1}{r(V)^2}.
\ee
We can now see that the integrand is linear in $p(V)$. To make the integral easier to digest, we let $V(x)=V_{max}$, and applying the asymptotically AdS condition \eqref{asymads}, we have
\be
\label{pV}
\D\p\left(\sqrt{V_{max}}\right) = \int^{V_{max}}_{1/R^2}\dfrac{p(V)\,\d V}{\displaystyle\sqrt{V_{max} - V}}.
\ee
It is first noted that equation \eqref{pV} is an integral equation of the first kind. The simplest equation of this type is $a(x)=\int^x_0b(r)\,dr$, which has the trivial solution $b(r)=a^\prime(r)$. More precisely, equation \eqref{pV} is a Volterra equation of the First Kind. It is a particular form of the {\it generalized Abel equation} \cite{Abel}, which is of the form
\be
\int^x_a\dfrac{y(t)}{(x-t)^\lambda}\,dt=f(x),\quad 0<\lambda<1,
\ee
with solution,
\be
y(t)=\dfrac{\mathrm{sin}(\pi\lambda)}{\pi}\dfrac{d}{dt}\int_a^t\dfrac{f(x)\,dx}{(t-x)^{1-\lambda}}.
\ee
Applying this to equation \eqref{pV}, we have,
\be
p(V)=\dfrac{1}{\pi}\dfrac{d}{dV}\int^{V}_{1/R^2}\dfrac{\D\p\left(\ds\sqrt{V_{max}}\right)\,dV_{max}}{\ds\sqrt{V-V_{max}}}.
\ee
Now substituting back in for the original variables,
\be
-2\,\dfrac{\d r}{\d V}\,r^{-2}=\dfrac{2}{\pi}\dfrac{d}{dV}\int^{\sqrt{V}}_{1/R}\dfrac{\a\,\D\p(\a)}{\ds\sqrt{V-\a^2}}\,\d\a.
\ee
Integrating up, and applying the boundary conditions $V(r)=V$ and $V(\infty)=1/R^2$, we finally arrive with,  
\be
\label{exfr}
\int^{\sqrt{V(r)}}_{1/R}\dfrac{\a\,\D\p(\a)}{\ds\sqrt{V(r)-\a^2}}\,\d\a-\dfrac{\pi}{r}=0.
\ee
Thus given the location of the endpoints of null geodesics by the function $\D t(\D\p)$, one can find $\D\p(\a)$ using equation \eqref{atodt}, and in principle, solve for the metric function\footnote{One can use the same method to recover $f(r)$ using $\D t(\a)$ instead via equation \eqref{dt}. In this case, using the same inversion techniques, we find
\be
\label{exfr2}
V(r)\int^{\sqrt{V(r)}}_{1/R}\dfrac{\D t(\a)}{\sqrt{V(r)-\a^2}}\,d\a-2\int^{\sqrt{V(r)}}_{1/R}\D t(\a)\sqrt{V(r)-\a^2}\,d\a-\dfrac{\pi}{r}=0
\ee} $f(r)=r^2V(r)$ using \eqref{exfr}. In the next section, we will define what we mean by ``in principle'' by analysing the method of extraction using test functions.

\section{Analysing the extraction} 

Before considering the limits of the extraction method, it is useful to check the validity of \eqref{exfr} in simple cases where $\D\p(\a)$ is known, namely AdS space

Given $f(r)=1+r^2/R^2$, we can show that $\D\p(\a)=\pi$. So subtituting this result into \eqref{exfr} we have,
\bea
\int^{\sqrt{V(r)}}_{1/R}\dfrac{\a}{\ds\sqrt{V(r)-\a^2}}\,d\a&=&\dfrac{1}{r}\nn
\Rightarrow \ds\sqrt{V(r)-\dfrac{1}{R^2}}&=&\dfrac{1}{r}\nn
\Rightarrow f(r)&=&r^2\,V(r)=1+\dfrac{r^2}{R^2}.
\eea
Thus \eqref{exfr} has reproduced the the known result for pure AdS space.

We can also test the extraction for a known perturbed AdS solution, namely the AdSBH. In this case we take the metric in \eqref{sm} with $f(r)=1+r^2-0.1/r^2$ (see figure \ref{BHplot}), use this to find a numerical solution for $\D\p(\a)$, and then numerically solve for $V(r)=f(r)/r^2$ using \eqref{exfr}. The result is shown in figure \ref{BHplotextr}. Here we find the first limitation of the extraction method outlined in the previous section. We see that the spacetime can only be probed down to the radius of null geodesics $r_m$. This makes sense as Type $\B$ geodesics do not exist for $J<E/\a_m$, where\footnote{see the argument in section \ref{btbngeo}} $\a_m=\sqrt{V(r_m)}$.
\begin{figure}
\label{BHplotextr}
\centering
\includegraphics[height=3in,width=5in]{BHnullextr}
\caption{This is a plot of $V(r)=1+1/r^2-0.1/r^4$ (blue), compared with the data extracted using \eqref{exfr} (red). Notice the spacetime can only be extracted up to the maximum of the potential at $r_m=\sqrt{0.2}$.} 
\end{figure}

Now we can analyse the extraction for a more general type of function $V(r)$. We do this by adding some gaussian ``bumps'' to an AdSBH solution so that
\be
\label{bumpyfr}
V(r)=\dfrac{f(r)}{r^2}=1+\dfrac{1}{r^2}-\dfrac{1}{5r^4}+\displaystyle\sum_{i=1}^3\dfrac{\mathrm{A_i}}{\sqrt{2\pi}\sigma_i}\,e^{-\frac{(r-\mu_i)^2}{2{\sigma_i}^2}},
\ee
where $\mathrm{A_i}=(0.05,0.03,0.1),\,\mu_i=(1,1.3,2)\,\,\text{and}\,\,\sigma_i=(0.1,0.1,0.3)$.
\begin{figure}
\label{BHbumpyextr}
\centering
\includegraphics[height=3in,width=5in]{BHbumpyextr}
\caption{This is a plot of $V(r)$ given in \eqref{bumpyfr} (blue), compared with the data extracted using \eqref{exfr} (red). Notice the spacetime can only be extracted up to the maximum of the potential at $r_m=\sqrt{0.4}$.} 
\end{figure}
The extrated data is given in figure \ref{BHbumpyextr}. Again, we have the same limitation that the metric can only be determined down to $r_m$, but the shape of $V(r)$ does not limit the extraction as long as $V(r)$ is monotonically decreasing for $r>r_m$.


\section{The Series Solution}

Now that we have an expression for the metric $f(r)$ in terms of $\D\p(\a)$, we can now start to look for general examples where the intergral in equation \eqref{exfr} can be solved analytically in the forn of a series solution. In this section we explore the limitations of such a process. 

\subsection{The method}
\label{pertmeth}

Given a generic function $\D\p(\a)$ which describes a perturbed AdS spacetime, we can always expand about the pure AdS solution $\D\p(\a)=\pi$ in a power series by introducing a parameter $\e>0$ such that
\be
\label{pertdp}
\D\p(\a)=\pi+\pi\sum_{n=1}^{\infty}a_n\e^n(\a^2-1/R^2)^{n/2}
\ee
The parameter $\e$ is a bookeeping tool to define the order of the perturbation, but its value is unimportant and will eventually be set to $1$.

From the energy equation of null geodesics,
\be
\dot{r}^2+V(r)=\a^2,
\ee
we have the boundary values $\a\tend\frac{1}{R}$ as $r\tend\infty$, and so equation \eqref{pertdp} has the correct boundary behaviour $\D\p(1/R)=\pi$, since all boundary null geodesics end at the anti-podal point.

We can then ansatz a power series solution
\be
\label{pertV}
V(r)=\dfrac{1}{r^2}+\dfrac{1}{R^2}+\sum_{n=1}^{\infty}\e^nV_n(r)
\ee
where we have expanded about the pure AdS potential $\dfrac{1}{r^2}+\dfrac{1}{R^2}$ in powers of $\e$. To have the correct AdS asymptotics (see \eqref{asymads}), $V_n(r)\sim\O(1/r^{d+1+n})$ for large $r$, where $d+2$ is the dimension of the spacetime.

One can now solve for the the functions $V_n(r)$ by substituting \eqref{pertdp} and \eqref{pertV} into \eqref{exfr}, and solving order by order in powers of $\e$.

Substituting \eqref{pertdp} into \eqref{exfr} and solving the integral, we have
\be
\sqrt{V(r)-\dfrac{1}{R^2}}+\dfrac{\sqrt{\pi}}{2}\sum_{n=1}^{\infty}a_n\e^n\dfrac{\G(\frac{2+n}{2})}{\G(\frac{3+n}{2})}\left(V(r)-\frac{1}{R^2}\right)^{\frac{n+1}{2}}=\dfrac{1}{r}
\ee
Now subtituting in the series \eqref{pertV}, and performing a Taylor series expansion about $\e=0$, we can solve for the functions $V_n(r)$ order by order in powers of $\e$. The first terms in the series are given by,
\bea
V_1(r)&=&-\dfrac{\pi}{2}a_1\dfrac{1}{r^3}\nn
V_2(r)&=&\left(\dfrac{5\pi^2}{16}a_1^2-\dfrac{4}{3}a_2\right)\dfrac{1}{r^4}\nn
V_3(r)&=&-\pi\left(\dfrac{7\pi^2}{32}a_1^3-2a_1a_2+\dfrac{3}{8}a_3\right)\dfrac{1}{r^5}\nn
&\vdots&\nn
V_n(r)&=&\dfrac{b_n(a_1,a_2,\cdots,a_n)}{r^{n+2}}.
\eea
By setting $\e=1$, we have the metric given as a power series solution,
\be
\label{fpert}
f(r)=\dfrac{r^2}{R^2}+1+\sum_{n=1}^\infty\dfrac{b_n}{r^n}.
\ee
The range of values of $r$ for which \eqref{fpert} is a good approximation of the actual geometry is determined by the convergence of the power series. Using the ratio test for convergence, we find the range of validity
\be
\label{convr}
\lim_{n\tend\infty}\left|\dfrac{b_{n+1}}{b_n}\right|<r<\infty.
\ee

Thus, given any boundary data for which the function $\D\p(\a)$ which can be written as the series given in \eqref{pertdp}, one can determine the geometry of the perturbed AdS bulk with metric \eqref{sm} over the region \eqref{convr} to good approximation.

\subsection{An Example: The ``star'' geometry}

In the previous section we described the general method for determining $f(r)$ as a series solution. In this section we will check the results with a known solution that behaves like the interior of a star\footnote{The geometry described here is a simplified version of the ``star'' geometry considered in \cite{hubeny}, where we have let the metric depend on one function only. See the referenced paper for an analysis of the full geometry}.

A class of boundary functions which model the angular seperation of the endpoints of Type $\B$ null geodesics in star geometries is given by (see fig \ref{starplot})
\be
\label{stardp}
\D\p(\a)=\pi+A\ds\sqrt{\a^2-\frac{1}{R^2}}\exp\left(-B\ds\sqrt{\a^2-\frac{1}{R^2}}\right),
\ee
where $R$ is the AdS radius, $\a=E/J$ and $A,B$ are aritrary positive constants. 

By performing a Taylor series expansion of \eqref{stardp} about $\sqrt{\a^2-1/R^2}=0$, we can reproduce the form of $\D\p$ given in \eqref{pertdp} with $\e=1$ and $a_n=\frac{A}{\pi}\frac{(-B)^{n-1}}{(n-1)!}$. One can then immediately use the method in the previous section to determine the constants $b_n$, such that the star metric $f(r)$ can be written as a series solution. The series solution is compared with the numerical solution for a specific case of \eqref{stardp} in figure \ref{starpertplot}. It illustrates that one can extract the metric function $f(r)$ perturbatively to high enough orders as long as the series is convergent. Given that the range of convergence is given by \eqref{convr}, and from the analysis of figure \ref{starpertconv}, we can make the approximation that $\lim_{n\tend\infty}|\frac{b_{n+1}}{b_n}|\sim A(1+B)$, the pertubative extraction using \eqref{stardp} is valid for
\be
A(1+B)\lesssim r<\infty.
\ee 

\begin{figure}[h!t]
\centering
\label{starplot}
\begin{tabular}{cc}
\begin{minipage}{225pt}
\centerline{\includegraphics[width=225pt]{stardp}}
\end{minipage}
&
\begin{minipage}{225pt}
\centerline{\includegraphics[width=225pt]{stardtdp}}
\end{minipage}
\end{tabular}
\caption{To the left is a plot of $\D\p$ given in \eqref{stardp} for $A=R=1$ and $B=\{0.2,0.3,0.5,1\}$. We see the correct boundary behaviour where $\D\p(1)=\pi$. We also notice that as $\a\tend\infty,\,\,\D\p\tend\pi$. This represents the behaviour of radial null geodesics where $J\tend 0$. To the right is a plot of $\D t(\D\p)$ by using the relation \eqref{atodt} on the $\D\p(\a)$ curves in the left plot. We see as $\D t,\D\p\tend\pi$ we recover the behaviour of Type $\A$ boundary null geodesics $\D t=\D\p$. For radial null geodesics we see a shift in $\D t$ due to the presence of matter in the bulk. These plots are very similar to the full star geometry shown in \cite{hubeny}, and so we are justified in using the expression for $\D\p(\a)$ given in \eqref{stardp}}
\end{figure}

\begin{figure}
\label{starpertplot}
\centering
\includegraphics[height=3in,width=5in]{starpert}
\caption{Here we compare the perturbative solution of \eqref{fpert} given the boundary function $\D\p$ in \eqref{pertdp} with $A=0.5$ and $B=0.1$, to the actual geometry solved numerically (shown in black). The order $n$ of the perturbation is given by $(n=1)=\,$Purple, $(n=2)=\,$Blue, $(n=10)=\,$Green, $(n=25)=\,$Red. The pure AdS metric with radius $R=1$ is given by the dashed line. We see that for $r\gg R$, all solutions tend to the AdS solution, which must be true by construction. For increasing order $n$, the series solution converges to the numerical solution for $r\gtrsim 0.6$.} 
\end{figure}

\begin{figure}
\label{starpertconv}
\centering
\includegraphics[height=3.5in,width=5in]{starpertconv}
\caption{This plot shows the absolute value of the ratio of coefficients $b_{n+1}/b_n$ of the series \eqref{fpert} for increasing number of terms $n$. The series shown in figure \ref{starpertplot} is represented by the red points, with similar series solutions given by $(A=1,B=0.1)=\,$Blue, $(A=1,B=0.2)=\,$Yellow, $(A=1,B=1)=\,$Green. We see that the quantity $\lim_{n\tend\infty}|\frac{b_{n+1}}{b_n}|$ exists for all values of $A$ and $B$, where $\lim_{n\tend\infty}|\frac{b_{n+1}}{b_n}|\sim A(1+B)$.} 
\end{figure}

\subsection{Recovering the AdSBH solution}

An alternative approach to check the consistancy of the perturbation is to start with a known metric function and recover the boundary function which reproduces it as a series. This can then be compared with the numerical result.

The AdSBH in $d+1$ dimensions ($d>2$) has metric \eqref{sm}, where
\be
f(r)=\dfrac{r^2}{R^2}+1-\dfrac{r_+^{d-2}}{r^{d-2}}\left(1+\dfrac{r_+^2}{R^2}\right).
\ee
Comparing this with \eqref{fpert}, we can match the terms by setting $b_{n\neq d-2}=0$. This is achieved perturbatively by setting $a_{0<n<d-2}=0$ and picking $a_{n>d-2}$ such that $b_{n>d-2}=0$. Using the results in section \ref{pertmeth}, and setting $\e=1$ as before, we have
\be
f(r)=\dfrac{r^2}{R^2}+1+\dfrac{b_{d-2}}{r^{d-2}},
\ee
where
\be
b_{d-2}=-a_{d-2}\sqrt{\pi}\dfrac{\G(\frac{d}{2})}{\G(\frac{d+1}{2})}.
\ee
Comparing with the AdSBH metric, we have
\be
\label{mcoef}
a_{d-2}=\dfrac{r_+^{d-2}}{\sqrt{\pi}}\dfrac{\G(\frac{d+1}{2})}{\G(\frac{d}{2})}\left(1+\dfrac{r_+^2}{R^2}\right).
\ee
The other non-zero coefficients such that $b_{n\neq d-2}=0$ are $a_{p(d-2)}$ where $p\in\mathbb{N}$. The first few are given by,
\bea
a_{2(d-2)}&=&\dfrac{(2d-1)}{4}\dfrac{r_+^{2(d-2)}}{\sqrt{\pi}}\dfrac{\G(\frac{2d-1}{2})}{\G(d-1)}\left(1+\dfrac{r_+^2}{R^2}\right)^2\nn
a_{3(d-2)}&=&\dfrac{(1-4d+3d^2)}{8}\dfrac{r_+^{3(d-2)}}{\sqrt{\pi}}\dfrac{\G(\frac{3d-3}{2})}{\G(\frac{3d-4}{2})}\left(1+\dfrac{r_+^2}{R^2}\right)^3\nn
\vdots\nn
a_{p(d-2)}&=&P_{p-1}(d)\dfrac{r_+^{p(d-2)}}{\sqrt{\pi}}\dfrac{\G(\frac{3+p(d-2)}{2})}{\G(\frac{2+p(d-2)}{2})}\left(1+\dfrac{r_+^2}{R^2}\right)^p,
\eea
where $P_{p-1}(d)$ is an order ${p-1}$ polynomial in $d$.

Now we can determine the range of $\a$ for which the expansion of $\D\p(\a)$ given in \eqref{pertdp} is convergent. Using the ratio test, we have
\be
\dfrac{1}{R^2}<\a^2<\dfrac{1}{R^2}+\lim_{p\tend\infty}\left|\dfrac{a_{p(d-2)}}{a_{(p+1)(d-2)}}\right|^\frac{2}{d-2}.
\ee
For large $p$, we can make the approximation $P_{p-1}(d)\sim d^{p-1}$, so substituting for the coefficients $a_{p(d-2)}$, the convergence condition reduces to
\be
\dfrac{1}{R}<\a\lesssim\dfrac{1}{R}\ds\sqrt{1+\dfrac{R^2}{r_+^2}\left[d\left(1+\dfrac{r_+^2}{R^2}\right)\right]^{-\frac{2}{d-2}}}.
\ee
Thus for a small black hole where $r_+<R$, the range of $\a$ for which the series \eqref{pertdp} is a good approximation, is larger than for a large black hole where $r_+>R$. This reflects the fact that for a large black hole, the geometry is more perturbed, so the expansion around AdS will probe smaller distances away from the boundary. The range of $\a$ is also limited by a physical upper bound set by the radius of null circular orbits $r_m$. Type $\B$ null geodsics entering the region $r<r_m$ do not return to the boundary due to the presence of the singularity. In the specific case of the AdSBH, $r_m$ is determined by the the global maximum of the potential $V(r)=f(r)/r^2$, and so
\be
\dfrac{dV(r)}{dr}\Big|_{r=r_m}=0\quad\thus r_m=r_+\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{1}{d-2}.
\ee
The value of $\a$ at $r=r_m$ is given by the energy condition,
\bea
\a_m^2=V(r_m)&=&\dfrac{1}{R^2}+\left(\dfrac{d-2}{d}\right)\dfrac{1}{r_m^2}\nn
&=&\dfrac{1}{R^2}+\left(\dfrac{d-2}{d}\right)\dfrac{1}{r_+^2}\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{2}{2-d},
\eea
and so the range of $\a$ which parametrises Type $\B$ null geodesics in a $d+1$ dimensional AdSBH is given by
\be
\dfrac{1}{R}<\a<\dfrac{1}{R}\sqrt{1+\left(\dfrac{d-2}{d}\right)\dfrac{R^2}{r_+^2}\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{2}{2-d}}.
\ee
And so, we see that the power series \eqref{pertdp} is convergent for the entire physical range of $\a$ when
\bea
\dfrac{1}{R}\sqrt{1+\left(\dfrac{d-2}{d}\right)\dfrac{R^2}{r_+^2}\left[\dfrac{d}{2}\left(1+\dfrac{r_+^2}{R^2}\right)\right]^\frac{2}{2-d}}&\lesssim&\dfrac{1}{R}\ds\sqrt{1+\dfrac{R^2}{r_+^2}\left[d\left(1+\dfrac{r_+^2}{R^2}\right)\right]^{-\frac{2}{d-2}}}\nn
\thus d&\gtrsim&4.
\eea
This is illustrated in figure \ref{BHpert} for $d=4$.
\begin{figure}
\label{BHpert}
\centering
\includegraphics[height=3.5in,width=5in]{BH_pert}
\caption{Here are graphs of $\D\p(\a)$ given an AdSBH spacetime with metric $f(r)=1+r^2-\m/r^2$ with $\m=0.3$ (left) and $0.1$ (right). The numerical result is shown in black and is compared with the perturbative solutions with increasing order $n=\{1,2,5,10,20\}$. We see that for large enough orders, the series given in \eqref{pertdp} can recover the AdSBH metric up to the radius of null circular orbits $r_m=\sqrt{2\m}$.} 
\end{figure}

\section{Summery}
In this chapter we have shown how one can extract a special class of asymptotically AdS metrics \eqref{sm}, given the location of singular correlation functions in the dual boundary CFT. This was achieved via an integral inversion and was verified using known cases. The limitations of such an extraction were discussed, and it was shown that for spacetimes admitting a singularity at the origin, the metric function could only be determined down to the radius of null circular orbits. Extracting the metric as a series solution was also investigated, and a general method was discovered. This was again tested using some known examples.

In the next chapter we will investigate a more general class of spacetimes where there are two unknown metric functions. In this case the knowledge of the location of the endpoints of Type $\B$ null geodesics will not be enough to determine the metric. One will require the knowledge of the entanglement entropy in special subsets of the boundary CFT manifold as mentioned at the beginning of this chapter.  

\newpage

